Described Object Detection: Liberating Object Detection with Flexible Expressions

Detecting objects based on language information is a popular task that includes Open-Vocabulary object Detection (OVD) and Referring Expression Comprehension (REC). In this paper, we advance them to a more practical setting called Described Object Detection (DOD) by expanding category names to flexible language expressions for OVD and overcoming the limitation of REC only grounding the pre-existing object. We establish the research foundation for DOD by constructing a Description Detection Dataset ($D^3$). This dataset features flexible language expressions, whether short category names or long descriptions, and annotating all described objects on all images without omission. By evaluating previous SOTA methods on $D^3$, we find some troublemakers that fail current REC, OVD, and bi-functional methods. REC methods struggle with confidence scores, rejecting negative instances, and multi-target scenarios, while OVD methods face constraints with long and complex descriptions. Recent bi-functional methods also do not work well on DOD due to their separated training procedures and inference strategies for REC and OVD tasks. Building upon the aforementioned findings, we propose a baseline that largely improves REC methods by reconstructing the training data and introducing a binary classification sub-task, outperforming existing methods. Data and code are available at https://github.com/shikras/d-cube and related works are tracked in https://github.com/Charles-Xie/awesome-described-object-detection.

==> figures/qualitative.tex <==
\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Visualization of the prediction results by different baseline methods on some samples from the proposed dataset.\Todo{pick case.}}
\label{fig:qualitative}
\end{figure}


==> tables/baselines.tex <==
\begin{table}[t]
    \centering
    \caption{Summarization and comparison of the baselines evaluated on the proposed benchmark.\Todo{add their performance on original tasks.}
    }
    \begin{tabular}{l | l | c c c c}
        % \hline
        Task & Method & Training Data & Framework \\
        \hline
        \hline
        REC & OFA & REC,OD, IC, VQA, MLM & Seq2seq \\
        \hline
        OVD & OWL-ViT & ITC, OD & ViT \\
        \hline
        Bi-functional & UNINEXT & OD, REC, Tracking, Segmentation & DETR \\
        Bi-functional & G-DINO & OD, REC, PG, IC & DETR \\
        \hline
        DOD & OFA-DOD & REC, OD, IC, VQA, MLM & Seq2seq \\
        % \hline
    \end{tabular}
    \label{tab:baselines}
\end{table}

